Weak gravitational lensing measurements of Abell 2744 using JWST and shear measurement algorithm pyRRG-JWST

We update the publicly available weak lensing shear measurement algorithm pyRRG for the James Webb Space Telescope, and apply it to UNCOVER DR1 imaging of galaxy cluster Abell 2744. At short wavelengths (< 2.5$\mu$m), shear measurements are consistent between independent observations through different JWST bandpasses, and calibrated within 1.5% of those from the Hubble Space Telescope. At longer wavelengths, shear is underestimated by ~5%, probably due to coarser pixellisation. We model the spatially varying Point Spread Function (PSF) using WebbPSF, whose moments are within 0.05 of real stars near the centre of the mosaic, where there are sufficient stars to also generate an empirical model. We measure shear from up to 162 galaxies arcminute$^2$ to derive a map of (dark plus baryonic) mass with 12 arcsecond (55 kpc) spatial resolution. All code, catalogues and maps are available from https://github.com/davidharvey1986/pyRRG.

==> results.tex <==
\begin{table*}
\begin{center}
\caption{\label{tab:haloStats}}
\begin{tabular}{cccccccc}
\hline
Model&$H_0/($km s$^{-1}$Mpc$^{-1}$)&$z_{lens}$&$\alpha$&log$(M(<5$kpc$)/M_\odot)$&$\Omega_M$&$\Omega_\Lambda$&$\Omega_K$\\
\hline
Fixed& $ 70_{-2}^{+2} $ & $ 0.36_{-0.04}^{+0.09} $ & $ -1.9_{-0.08}^{+0.08} $ & $ 11_{-0.2}^{+0.04} $ \\ 
$\Lambda$CDM& $ 71_{-3}^{+2} $ & $ 0.36_{-0.09}^{+0.2} $ & $ -1.8_{-0.1}^{+0.08} $ & $ 11_{-0.08}^{+0.1} $ & $ 0.3_{-0.04}^{+0.04} $ & $ 0.7_{-0.04}^{+0.04} $ \\ 
$\Lambda$CDMk& $ 71_{-3}^{+3} $ & $ 0.36_{-0.07}^{+0.2} $ & $ -1.8_{-0.1}^{+0.08} $ & $ 11_{-0.08}^{+0.1} $ & $ 0.3_{-0.05}^{+0.05} $ & $ 0.7_{-0.05}^{+0.05} $ & $ 0.00029_{-0.02}^{+0.02} $ \\ 
\hline
\end{tabular}
\end{center}
\end{table*}


==> table-1.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
Sample & $\epsilon$ (kpc / h ) &$\sigma_{DM}/m$ (cm$^2$/g) &$N_{\rm cl}$ & $N_{\rm eff}$ &\textcolor{red}{$\langle \log_{10} M_{\rm tot}/M_{\odot}\rangle$ or $\log_{10} \langle M_{\rm tot}/M_{\odot}\rangle$} \\
\hline
CDM & 4 & 0.0 & 1366 &  466 & 14.45 \\ 
SIDM0.1 & 4 & 0.1 & 1344 &  731 & 14.32 \\ 
SIDM0.3 & 4 & 0.3 & 1374 &  672 & 14.42 \\ 
SIDM & 4 & 1.0 & 1330 &  644 & 14.40 \\ 
CDM-hires & 2 & 0.0 &   80 &   13 & 14.23 \\ 
SIDM-hires & 2 & 1.0 &   95 &   18 & 14.25 \\ 
obs & 0 & 0.0 &   10 &   10 & 15.08 \\ 
\hline
\end{tabular}
\caption{ The sample selection of galaxy clusters from the simulations with their corresponding dark matter cross-section. The third column gives the total number of clusters extracted from the simulation and the fourth column gives the number of relaxed clusters after cuts. The final column gives the mean halo mass of the cut sample.
\label{tab:data}}
\end{table*}

